Inductive Meta-path Learning for Schema-complex Heterogeneous Information Networks

Heterogeneous Information Networks (HINs) are information networks with multiple types of nodes and edges. The concept of meta-path, i.e., a sequence of entity types and relation types connecting two entities, is proposed to provide the meta-level explainable semantics for various HIN tasks. Traditionally, meta-paths are primarily used for schema-simple HINs, e.g., bibliographic networks with only a few entity types, where meta-paths are often enumerated with domain knowledge. However, the adoption of meta-paths for schema-complex HINs, such as knowledge bases (KBs) with hundreds of entity and relation types, has been limited due to the computational complexity associated with meta-path enumeration. Additionally, effectively assessing meta-paths requires enumerating relevant path instances, which adds further complexity to the meta-path learning process. To address these challenges, we propose SchemaWalk, an inductive meta-path learning framework for schema-complex HINs. We represent meta-paths with schema-level representations to support the learning of the scores of meta-paths for varying relations, mitigating the need of exhaustive path instance enumeration for each relation. Further, we design a reinforcement-learning based path-finding agent, which directly navigates the network schema (i.e., schema graph) to learn policies for establishing meta-paths with high coverage and confidence for multiple relations. Extensive experiments on real data sets demonstrate the effectiveness of our proposed paradigm.

==> Section/ablation.tex <==
\section{Ablation Studies}
In this section, we carry out ablation studies to help comprehend the contribution of model components. Specifically, we vary the representations of entity type and the meta-path similarity function, and proceed the experiments on Yago. The result tables are placed in Appendix \ref{appendix:ablation}.

\subsection{Different Representations of Type Node}
\label{abl:emb}
\lsx{As noted above, we obtain and fix the type node embeddings with mean-pooling over the TransE-initialised entity embeddings. We here study the 
influence of 1) tuning and 2) entity embeddings initialisation, on~\model. For the former, with tuning, the type node embeddings of~\model~could be fine-tuned during training. For the latter, apart from TransE, we consider pRotatE and random initialisation. We adopt pRotatE, the variant proposed along with RotatE~\cite{sun2019rotate}, since the network topology of~\model only accepts entity/relation embeddings of the same dimension. In all, there are six type representation plans to compare.}
%For the latter, since RotatE produces better embeddings for representation than TransE in various downstream tasks~\cite{sun2019rotate}, we add it for comparison. We adopt pRotatE, a variant proposed along with RotatE, since the network topology of~\model\ only accepts entity/relation embeddings of the same dimension. We also consider random initialization with/without tuning as alternative plans.


As shown in Table \ref{table_abl_emb}, the choice of TransE without tuning performs the best with decent prediction accuracy and search efficiency. Random initialization brings some fascinating results at the sacrifice of computation (nearly explored twice as many meta-paths compared with TransE). By contrast, pRotatE does not fit in well and delays the meta-path-finding process as its mechanism to embed entities and relations does not comply with \model's distance measure. On the other hand, tuning could improve the search efficiency of \model, but only if the embeddings are unsuitably initialised. If \model is equipped with an appropriate embedding like TransE, tuning disturbs the discovery process by constantly adjusting its type representation.

\subsection{Different Meta-path Similarity Functions}
\label{abl:sim}
%We also study the influence of meta-path similarity functions (i.e. the way to compute the similarity of two entities given meta-paths) on \model. 
\lsx{The meta-path similarity function gives the way to compute the similarity of two entities with various meta-paths.}
% We also study the influences of similarity models on \model. We fix the meta-paths discovered by \model\ and calculate similarities w.r.t different models accordingly.
Previously, we adopt the sum of confidence (\textit{Sum Conf.}) of meta-paths connecting two entities to measure similarity, and we here compare it with meta-path count (\textit{Meta. Count}), confidence features (\textit{Conf. Feat.}) and binary features (\textit{Binary Feat.}). The \textit{Meta. Count} is the number of meta-paths that traverse the pairs. The \textit{Binary Feat.} is a binary vector whose elements represent the connectivity of meta-paths between the pairs. The \textit{Conf. Feat.} replaces each positive element in the \textit{Binary Feat.} with the confidence of relevant meta-path. For the last two functions, the linear regression model known as LASSO could automatically select features, calculate the weight and return similarities. As shown in Table \ref{table_abl_simmodel}, it is intuitive that \textit{Sum Conf.} performs better than \textit{Meta. Count}, since different meta-path possesses different confidence level. The reason that \textit{Sum Conf.} and \textit{Meta. Count} outperform \textit{Conf. Feat.} and \textit{Binary Feat.} is that they free the regression model from the need to determine weights for each feature.


==> Tables/table_ablation.tex <==
\section{Further Results for Ablation Studies}
See Table \ref{table_abl_emb} and \ref{table_abl_simmodel} for the performance and efficiency of \model~with different entity embedding models and meta-path similarity functions, respectively.
\label{appendix:ablation}
\begin{table*}[h!]
    \centering
       \caption{Performance of different instance entity embedding models averaged over 5 times. The best and second best results for ROC-AUC/AP are marked in bold and underlined respectively. Metapath Explored denotes the number of meta-paths the agent needs to explore to find rewarding meta-paths during training.}
\resizebox{\linewidth}{!}{%
 \begin{tabular}{cc|c|c|c|c|c|c}
    \toprule[1.5pt]
   &&TransE&TransE with tuning&pRotatE&pRotatE with tuning&Random&Random with tuning
   \\
                 \hline
      \multirow{3}{*}{isCitizenOf}&ROC-AUC&\underline{${0.914\pm0.035}$}&$0.883\pm0.037$&$0.766\pm0.037$&$0.847\pm0.048$&$\pmb{0.916\pm0.034}$&$0.845\pm0.054$
       \\
       &AP&\underline{${0.927\pm0.029}$}&$0.913\pm0.032$&$0.838\pm0.032$&$0.903\pm0.030$&$\pmb{0.937\pm0.033}$&$0.902\pm0.038$
      \\
       &Metapath Explored&$909\pm137$&$811\pm100$&$218\pm35$&$888\pm269$&$2396\pm230$&$1151\pm56$
      \\
                   \hline
      \multirow{3}{*}{DiedIn}&ROC-AUC&\underline{${0.870\pm0.032}$}&$0.864\pm0.045$&$0.552\pm0.031$&$0.839\pm0.055$&$\pmb{0.896\pm0.044}$&$0.847\pm0.022$
       \\
       &AP&$\pmb{0.930\pm0.040}$&$0.905\pm0.047$&$0.687\pm0.067$&$0.869\pm0.036$&\underline{${0.909\pm0.050}$}&$0.872\pm0.037$
      \\
       &Metapath Explored&$4001\pm269$&$4823\pm1302$&$435\pm19$&$1140\pm309$&$7868\pm804$&$5674\pm1064$
      \\
                   \hline
      \multirow{3}{*}{GraduatedFrom}&ROC-AUC&\underline{${0.905\pm0.012}$}&$0.872\pm0.076$&$0.605\pm0.070$&$0.804\pm0.104$&$0.880\pm0.039$&$\pmb{0.917\pm0.056}$
       \\
       &AP&\underline{${0.939\pm0.039}$}&$0.904\pm0.064$&$0.722\pm0.047$&$0.871\pm0.081$&$0.927\pm0.028$&$\pmb{0.948\pm0.040}$
      \\
       &Metapath Explored&$1620\pm809$&$2534\pm962$&$117\pm33$&$2136\pm899$&$4786\pm1528$&$3331\pm839$
      \\
       \bottomrule[1.5pt]
   \end{tabular}
   }
   \label{table_abl_emb}
\end{table*}


\begin{table*}[h!]
    \centering
       \caption{Performance of different meta-path similarity functions averaged over 5 times. The bold results indicate the best ones among all functions for each relation.}
 \resizebox{0.65\linewidth}{!}{
 \begin{tabular}{cc|c|c|c|c}
    \toprule[1.5pt]
   &&\textit{Sum Conf.} &\textit{Meta. Count} &\textit{Conf. Feat.} &\textit{Binary Feat.}
   \\
                 \hline
      \multirow{2}{*}{isCitizenOf}&ROC-AUC&$\pmb{0.923\pm0.027}$&$0.917\pm0.035$&$0.812\pm0.048$&$0.802\pm0.031$
       \\
       &AP&$\pmb{0.955\pm0.011}$&$0.947\pm0.022$&$0.911\pm0.031$&$0.903\pm0.015$
      \\
                   \hline
      \multirow{2}{*}{DiedIn}&ROC-AUC&$\pmb{0.867\pm0.033}$&$0.853\pm0.032$&$0.837\pm0.028$&$0.833\pm0.035$
       \\
       &AP&$\pmb{0.931\pm0.038}$&$0.929\pm0.039$&$0.928\pm0.023$&$0.917\pm0.034$
      \\
                   \hline
      \multirow{2}{*}{GraduatedFrom}&ROC-AUC&$\pmb{0.919\pm0.015}$&$0.911\pm0.019$&$0.801\pm0.059$&$0.814\pm0.033$
       \\
       &AP&$\pmb{0.952\pm0.003}$&$0.945\pm0.015$&$0.885\pm0.040$&$0.890\pm0.034$
      \\
       \bottomrule[1.5pt]
   \end{tabular}
}
   \label{table_abl_simmodel}
\end{table*}
